Diamond-loaded polyimide aerogel scattering filters and their applications in astrophysical and planetary science observations

Infrared-blocking, aerogel-based scattering filters have a broad range of potential applications in astrophysics and planetary science instruments in the far-infrared, sub-millimeter, and microwave regimes. This paper demonstrates the ability of conductively-loaded, polyimide aerogel filters to meet the mechanical and science instrument requirements for several experiments, including the Cosmology Large Angular Scale Surveyor (CLASS), the Experiment for Cryogenic Large-Aperture Intensity Mapping (EXCLAIM), and the Sub-millimeter Solar Observation Lunar Volatiles Experiment (SSOLVE). Thermal multi-physics simulations of the filters predict their performance when integrated into a cryogenic receiver. Prototype filters have survived cryogenic cycling to 4\,K with no degradation in mechanical properties. Measurement of total hemispherical reflectance and transmittance, as well as cryogenic tests of the aerogel filters in a full receiver context, allow estimates of the integrated infrared emissivity of the filters. Knowledge of the emissivity will help instrument designers incorporate the filters into future experiments in planetary science, astrophysics, and cosmology.

==> old-text.tex <==

%\section{Diamond-loaded Polyimide Aerogel Design Parameters}
%\label{sec:design}
%\subsection{Aerogel Filter Design Principles}
%The diamond particle size and loading density are varied in order to tune the filter to the desired cutoff frequency. Particle size has the strongest effect on cutoff frequency. Larger particles have a lower cut-off frequency and smaller particles have a higher cut-off frequency. Diamond powders used typically have a Gaussian size distribution with the named range, e.g. 3-6 \textmu m, representing the 3-$\sigma$ size range. Polyimide aerogel filters have been fabricated with a range of diamond loading densities ranging from 20\,mg/cc up to 100\,mg/cc. Loading densities significantly above 100\,mg/cc prevent proper polymerization and curing of the base aerogel. For a given particle size distribution, a higher loading density creates a filter with a lower cut-off frequency and vice versa. In general, the scattering cross-section of the diamond particles goes as the square of the particle radius (area $\propto r^2$) and mass density goes as the cube of particle radius (volume $\propto r^3$). In order to capture the effect of particle radius and loading density, a ``column density'' can be calculated, that represents the total area of scatterers per unit area. Multiple particle size distributions and densities can be mixed together, e.g. primarily using a higher density of larger particles to set the primary cut-off frequency and mixing in lower densities of smaller particles to control high frequency leakage. 

%Figure \ref{fig:vertical_casting} shows images of the vertical casting mold. 
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = \columnwidth]{images/vertical_mold_diagram.JPG}
%    \caption{Images of a large vertical film casting mold. The mold is constructed out of two large, rigid pieces of plastic with a controllable gap of approximately 1\,mm between them. Aerogel sol is poured into the mold and takes the rigid shape of the large mold. }
%    \label{fig:vertical_casting}
%\end{figure}

% \subsection{Total Hemispherical Measurements of Diamond-loaded Polyimide Aerogel Filters and Other Media}

% Measurements of the total hemispherical reflectance and transmission of a filter media allows the characterization of how much light is reflected by or transmitted through a sample at all angles, instead of just the light along the optical axis of the incoming beam. 

% Diamond-loaded polyimide aerogel filter samples along with other commercially prepared foam samples were measured using a Bruker FTS equipped with an integrating sphere reflectometer. Samples were mounted inside of the integrating sphere and illuminated with a beam of light. The scattered light was collected by the integrating sphere and measured by the detector. An analogous measurement was made to find the total hemispherical transmittance. Because these measurements were made with an FTS, transmittance and reflectance data are available as a function of frequency/wavelength of light. Figure \ref{fig:total_hemi} shows the total hemispherical data for the commercially available foam prodcuts as well as the Recipe G of the EXCLAIM formulation of the diamond-loaded aerogel filters. 

% An additional benefit making the total hemispherical measurements is that the emissivity can be estimated by subtracting the sum of the reflectance and transmittance from unity:
% \begin{equation}
%     \epsilon \simeq 1  - T - R.
%     \label{eqn: emissivity}
% \end{equation}
% Figure \ref{fig:total_hemi} shows the estimated emissivity for the various samples across a broad range of frequencies. The white Zotefoam samples have a substantially lower estimated emissivity than the black foams, the polystyrene foam, and the aerogel filter. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width = \columnwidth]{images/THT-foams_ag.eps}
%     \includegraphics[width = \columnwidth]{images/THR-foams_ag.eps}
%     \includegraphics[width = \columnwidth]{images/emissivity-foams_ag.eps}
%     \caption{\textit{Top:} \textit{Bottom:} Comparison of the transmittance of different infrared filters. The Zotefoam filter and XPS foams are shown for a filter 3\,mm thick. The Zitex is shown for a filter that is 0.1\,mm thick. The diamond-loaded polyimide aerogel filter is loaded with 60\,mg/cc of 10-20~\textmu m and 40\,mg/cc of 3-6~\textmu m particles, and is a sample that is 0.18\,mm thick. The IR shader is 0.004\textmu m thick. The white LD24 and HD30 samples show higher transmission than the other samples, which leads to a lower calculated emissivity.}
%     \label{fig:total_hemi}
% \end{figure}


